Brownian Motion, "Diverse and Undulating"

We describe in detail the history of Brownian motion, as well as the contributions of Einstein, Sutherland, Smoluchowski, Bachelier, Perrin and Langevin to its theory. The always topical importance in physics of the theory of Brownian motion is illustrated by recent biophysical experiments, where it serves, for instance, for the measurement of the pulling force on a single DNA molecule. In a second part, we stress the mathematical importance of the theory of Brownian motion, illustrated by two chosen examples. The by-now classic representation of the Newtonian potential by Brownian motion is explained in an elementary way. We conclude with the description of recent progress seen in the geometry of the planar Brownian curve. At its heart lie the concepts of conformal invariance and multifractality, associated with the potential theory of the Brownian curve itself.

==> bourbaphyBEdefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin of definition file AHPEFS.TEX                      %
% (c) Stephan Ammann, for Birkhaeuser, Dec 1999            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AHPDEFS.tex -- is red in by each header file             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\font\fxtit=cmssbx10 % For the new logo

\newcount\fpage\newcount\npage\newcount\lpage
\fpage=\fipage\npage=\nrpage
\lpage=\fpage\advance\lpage by\npage\advance\lpage by-1

\def\xrule{\vrule width2.25pt}
\def\yrule{\hrule height.5pt}
\def\yrulefill{\leaders\yrule\hfill}
\def\strutx{\vrule height8.5pt width0pt depth0pt}
\def\struty{\vrule depth3.5pt width0pt}
\def\strutz{\vrule height10.2pt width0pt}

\def\boxl{\vbox{\halign{##\hfil\cr
{\sc Einstein, 1905-2005},
Poincar{\'e} Seminar \volnr\ (\centnr\yearnr)\cr
T. Damour, O. Darrigol, B. Duplantier \& V. Rivasseau, {eds.}\cr
{\it Progress in Mathematical Physics}, Vol. 47, \the\fpage\ -- \the\lpage\cr
\struty
%\copyright\
Birkh{\"a}user Verlag, Basel,
\centnr 06\cr
}}}


\def\boxr{\vbox{\offinterlineskip
\halign{##\hfil\hskip1mm&##\hfil\cr
\noalign{\vskip.8mm}
\multispan2{\yrulefill}\cr
\xrule\strutz\struty
&\fxtit Poincar{\'e} Seminar 2005 \cr
%\xrule\strutx&%
%\vbox to0pt{%
%\vbox to0pt{\vss\hbox{\fxtit and Applications NoDEA}}\vss}\cr
}}}

\def\titlebox{\vbox to0pt{\hsize=125mm\footnotesize\vss
\hbox to\hsize{\boxl\hfil\boxr}}}


\def\ps@myheadings{
\let\@mkboth\markboth
\def\@oddhead{\footnotesize \rm Vol. \volnr, \centnr\yearnr
\hspace{6mm}\titletxt\hfil\thepage}%
\def\@oddfoot{} % % centered page number
\def\@evenhead{\footnotesize \thepage \hfil
\authortxt\hspace{6mm}Poincar{\'e} Seminar 2005}%
\def\@evenfoot{}%       % centered page number
}

\def\ps@plain{
\let\@mkboth\markboth
\def\@oddhead{%
\titlebox}%
\def\@oddfoot{}%      % centered page number
\def\@evenhead{}%
\def\@evenfoot{}%     % centered page number
}

\ps@myheadings              % 'myheading' page style
\pagenumbering{arabic}      % Arabic page numbers
\onecolumn                  % Single-column.

\setcounter{page}{\fpage}

\textwidth=125mm
\textheight=185mm
\parindent=8mm
\evensidemargin=0pt
\oddsidemargin=0pt
\topmargin=0pt
\frenchspacing

\newcommand{\pdpg}{\postdisplaypenalty=-2000}
%% Used to force a page-break after a displayed equation

\let\dst=\displaystyle
\let\scr=\scriptstyle

\def\bfdefault{b}

\def\Rec{Received\ }
\def\Rev{Revised\ }

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of AHPDEFS.TEX                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of definition file

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% TeX-master: t
%%% TeX-master: t
%%% End: 

